Automatic Quantization for Physics-Based Simulation

Quantization has proven effective in high-resolution and large-scale simulations, which benefit from bit-level memory saving. However, identifying a quantization scheme that meets the requirement of both precision and memory efficiency requires trial and error. In this paper, we propose a novel framework to allow users to obtain a quantization scheme by simply specifying either an error bound or a memory compression rate. Based on the error propagation theory, our method takes advantage of auto-diff to estimate the contributions of each quantization operation to the total error. We formulate the task as a constrained optimization problem, which can be efficiently solved with analytical formulas derived for the linearized objective function. Our workflow extends the Taichi compiler and introduces dithering to improve the precision of quantized simulations. We demonstrate the generality and efficiency of our method via several challenging examples of physics-based simulation, which achieves up to 2.5x memory compression without noticeable degradation of visual quality in the results. Our code and data are available at https://github.com/Hanke98/AutoQuantizer.

==> tables/error_compare_table.tex <==
% Please add the following required packages to your document preamble:
% 

\begin{table*}%[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|l|l|l|l|l|l|l|l|l}
\hline
\textbf{Exp}   & \textbf{Steps/Frame} & \textbf{Frames} & \textbf{dt} & \textbf{Grids} & \textbf{Particles} & \textbf{Activated Cells} & Memory Compression Rate & \textbf{Target Error Bound} & \textbf{Errors} \\ \hline
Smoke 2D       &                      &                 &             &                &                    &                          &                         &                             &                 \\ \hline
Smoke 3D       &                      &                 &             &                &                    &                          &                         &                             &                 \\ \hline
MPM 2D Elastic &                      &                 &             &                &                    &                          &                         &                             &                 \\ \hline
MPM 3D Elastic &                      &                 &             &                &                    &                          &                         &                             &                 \\ \hline
MPM 2D Fluid   &                      &                 &             &                &                    &                          &                         &                             &                 \\ \hline
MPM 3D Fluid   &                      &                 &             &                &                    &                          &                         &                             &                 \\ \hline
\end{tabular}%
}
\end{table*}

==> tables/error_control_bak.tex <==
\begin{table}%[h]
    \caption{Results of the error-bounded experiments. The column of the control objective dictates the absolute tolerance of the simulation error. The quantized evaluation function lands nicely within the range of permitted error bound. Of all 160 experiments, there are 136 times that our quantization scheme manages to control the value.}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{c|c|c|c|c|c}

    \toprule
    \textbf{Exp.}     &{\textbf{\begin{tabular}[c]{@{}c@{}}Error \\ Tolerance ($\epsilon_{err}$)\end{tabular}}} & \textbf{ Control Objective } & \textbf{\begin{tabular}[c]{@{}c@{}}Quantized\\ Evaluation Function\end{tabular}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Success \\ Rate\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Compression\\ Rate\end{tabular}}} \\ \midrule \midrule
    \textbf{Exp. 1}    &0.1& $6.9 \pm 2.1 \times 10^3 $                        & $7.1  \pm 1.1 \times 10^3 $       & 19/20     & 2.00x  \\
    \textbf{Exp. 2}   &0.1& $1.87\pm 0.56\times 10^4 $                        & $3.69 \pm 0.08 \times 10^4 $         & 0/20   & 5.05x \\ \hline
    \textbf{Exp. 1}    &0.01& $6.89 \pm 0.21\times 10^3 $                      & $6.90 \pm 0.06 \times 10^3 $         & 20/20  & 1.67x \\
    \textbf{Case 2}   &0.01& $1.875\pm 0.056\times 10^4 $                     & $1.90 \pm 0.04 \times 10^4 $         & 17/20  & 3.20x \\ \hline
    \textbf{Exp. 1}     &0.001& $6.893 \pm 0.021\times 10^3 $                   & $6.895 \pm 0.008 \times 10^3 $        & 20/20   & 1.42x \\
    \textbf{Exp. 2}   &0.001& $1.8749\pm 0.0056\times 10^4 $                  & $1.875 \pm 0.003 \times 10^4 $         & 20/20   & 2.40x \\ \hline
    \textbf{Exp. 1}     &$1 \times 10^{-4}$ &$6.8934 \pm 0.0021\times 10^3$         & $6.8946 \pm 0.0007 \times 10^3 $       & 20/20   & 1.23x \\
    \textbf{Exp. 2}   &$1 \times 10^{-4}$ &$1.87486\pm 0.00056\times 10^4$        & $1.87488 \pm 0.00019 \times 10^4 $     & 20/20   & 1.96x \\ \bottomrule
    \end{tabular}
    }
    \label{tab:error-comparsion}
    \end{table}

    % \begin{table}[]
    % \caption{Per step running time of three different implementations, on CPUs and GPUs. The benchmark is initialized using a random pattern with $41690^{2}$ active cells with $50\%$ live cells. We run CPU benchmarks on an Intel i7 processor (six cores each at 2.6 GHz) and 16GB of memory. We run GPU benchmarks on an NVIDIA RTX 3080 GPU with 10GB of GPU memory.}

    % \centering
    % \resizebox{\linewidth}{!}{%
    % \begin{tabular}{c|c|c}
    % \toprule
    % \textbf{Implementation}    & \textbf{Time per step (CPU)} & \textbf{Time per step (GPU)} \\ \midrule \midrule
    % QuickLife                  & $318.5$ ms                      & N/A                          \\ \hline \hline
    % Non-vectorized brute-force & $9313.4$ ms                     & $546.0$ ms                      \\ \hline \hline
    % Vectorized brute-force     & $417.2$ ms                      & $3.4$ ms                        \\
    % \bottomrule
    % \end{tabular}%
    % }
    % \label{tab:gol-stat}
    % \end{table}
